Physics at Super B Factory

This report presents the results of studies that investigate the physics reach at a Super B factory, an asymmetric-energy e^+e^- collider with a design luminosity of 5 x 10^35 cm^-2s^-1, which is around 40 times as large as the peak luminosity achieved by the KEKB collider. The studies focus on flavor physics and CP violation measurements that could be carried out in the LHC era. The physics motivation, key observables, measurement methods and expected precisions are presented. The sensitivity studies are a part of the activities associated with the preparation of a Letter of Intent for SuperKEKB, which has been submitted recently.

==> sensitivity_dtaunu/defs-blife.tex <==
%======================= The results ==========================================
\def\tbzresultmean{1.554}
\def\tbzresultstat{\pm 0.030}
\def\tbzresultsyst{\pm0.019}

\def\tbmresultmean{1.695}
\def\tbmresultstat{\pm 0.026}
\def\tbmresultsyst{\pm 0.015}

\def\rbmresultmean{1.091}
\def\rbmresultstat{\pm 0.023}
\def\rbmresultsyst{\pm 0.014}

\def\yresultmean{0.114}
\def\yresultstat{{_{-0.064}^{+0.060}}}
\def\yresultsyst{{_{-0.011}^{+0.012}}}

\def\yinterval{-0.013 < y_{CP} < 0.234}

\def\tbzresult{\tbzresultmean \tbzresultstat\;\mbox{(stat)} \; \tbzresultsyst\;\mbox{(syst)}}
\def\tbmresult{\tbmresultmean \tbmresultstat\;\mbox{(stat)} \tbmresultsyst\;\mbox{(syst)}}
\def\rbmresult{\rbmresultmean \rbmresultstat\;\mbox{(stat)} \rbmresultsyst\;\mbox{(syst)}}
\def\yresult{\yresultmean \; \yresultstat \; \yresultsyst}

%%%

\def\rtau{r_\tau}

\def\yllimit{-0.36}
\def\yulimit{0.35}
\def\tbzdstlnu{1.50\pm0.06^{+0.06}_{-0.04}}
\def\tbmdstlnu{1.54\pm0.10^{+0.14}_{-0.07}}
\def\tbzdstpm{1.55^{+0.18}_{-0.17}{}^{+0.10}_{-0.07}}
\def\tbzdppm{1.41^{+0.13}_{-0.12}\pm0.07}
\def\tbmdzpm{1.73\pm0.10\pm0.09}
\def\tbmpsikm{1.87^{+0.13}_{-0.12}{}^{+0.07}_{-0.14}}
\def\tbzpsiks{1.54^{+0.28}_{-0.24}{}^{+0.11}_{-0.19}}
\def\tbzpsikst{1.56^{+0.22}_{-0.19}{}^{+0.09}_{-0.15}}
\def\Tbzdstlnu{$\taubz=(\tbzdstlnu)$~ps}
\def\Tbmdstlnu{$\taubm=(\tbmdstlnu)$~ps}
\def\Tbzdstpm{$\taubz=(\tbzdstpm)$~ps}
\def\Tbzdppm{$\taubz=(\tbzdppm)$~ps}
\def\Tbmdzpm{$\taubm=(\tbmdzpm)$~ps}
\def\Tbmpsikm{$\taubm=(\tbmpsikm)$~ps}
\def\Tbzpsiks{$\taubz=(\tbzpsiks)$~ps}
\def\Tbzpsikst{$\taubz=(\tbzpsikst)$~ps}
\def\Tbzresult{$\taubz=(\tbzresult)$~ps}
\def\Tbmresult{$\taubm=(\tbmresult)$~ps}
\def\Rbmresult{$\rbm=\rbmresult$}
\def\Yresult{$\ycp=\yresult$}
\def\Ylimit{$\yllimit<\ycp<\yulimit$}
\def\intl{5.1}

%========================= Commands ===========================================

\newcommand{\nim}[3]{Nucl. Inst. and Meth. {\bf #1} #2 (#3)}
\newcommand{\prld}[3]{Phys. Rev. Lett. {\bf #1} #2 (#3)}
\newcommand{\prdd}[3]{Phys. Rev. D {\bf #1} #2 (#3)}
\newcommand{\prxd}[3]{Phys. Rev. {\bf #1} #2 (#3)}
\newcommand{\plb}[3]{Phys. Lett. B {\bf #1} #2 (#3)}
\newcommand{\npa}[3]{Nucl. Phys. A {\bf #1} #2 (#3)}
\newcommand{\apphyslet}[3]{App. Phys. Lett. {\bf #1} #2 (#3)}
\newcommand{\zphysa}[3]{Z. Phys. A. {\bf #1} #2 (#3)}
\newcommand{\zpc}[3]{Z. Phys. C {\bf #1} #2 (#3)}
\newcommand{\jphys}[3]{J. Phys. {\bf #1} #2 (#3)}

%========================= deffinitions =======================================
\def\etal{{\it et al.}}
\def\chisqndf{{\chi}^2/n}
\def\chisq{\chi^2}
\def\Chisqndf{$\chisqndf$}
\def\Chisq{$\chisq$}
\def\NDF{$N.D.F.$}
\def\degree{{}^{\circ}}
\def\dG{\Delta\Gamma}
\def\dM{\Delta M}
\def\rmix{R_{\rm mix}}
\def\amix{A_{\rm mix}}
\def\re{{\cal R}e}
\def\im{{\cal I}m}
% \def\bzb{{\overline{B{}^0}}}
% \def\bb{{\overline{B{}^0}}}
\def\bzb{{\overline{B}{}^0}}
\def\bb{{\overline{B}{}^0}}
\def\kz{{K{}^0}}
\def\kzb{{\overline{K}{}^0}}
\def\kb{{\overline{K}{}^0}}
\def\bz{{B^0}}
\def\bh{{B_H}}
\def\bl{{B_L}}
\def\bm{{B^-}}
\def\bp{{B^+}}
\def\taubz{\tau(\bzb)}
\def\taubm{\tau(\bm)}
\def\rbm{\taubm/\taubz}
\def\Bzb{$\bzb$}
\def\Bm{$\bm$}
\def\Fb{fb$^{-1}$}
\def\ycp{y_{CP}}
\def\piz{\pi^0}
\def\pip{\pi^+}
\def\pim{\pi^-}
\def\kz{K^0}
\def\kp{K^+}
\def\km{K^-}
\def\ks{K_S^0}
\def\kl{K_L^0}
\def\kb{\overline{K}}
\def\rhom{\rho^-}
\def\bbar{\overline{B}}
\def\bbbar{B\bbar}
\def\bzbzbar{\bz\bzb}
\def\BBbar{$\bbbar$}
\def\BzBzbar{$\bzbzbar$}
\def\ccbar{c\overline{c}}
\def\CCbar{$\ccbar$}
\def\dstar{D^{*}}
\def\dstarz{{D^{*0}}}
\def\dstarp{D^{*+}}
\def\dstarzb{\overline{D}^{*0}}
\def\dstarm{D^{*-}}
\def\dmdstp{\Delta M_{\dstarp}}
\def\dmdstz{\Delta M_{\dstarz}}
\def\dmdst{\Delta M_{\dstar}}
\def\DM{$\Delta M$}
\def\Dstar{$\dstar$}
\def\Dstarz{$\dstarz$}
\def\Dstarp{$\dstarp$}
\def\Dstarzb{$\dstarzb$}
\def\Dstarm{$\dstarm$}
\def\nub{\overline{\nu}}
\def\jpsi{{J/\psi}}
\def\dz{D^0}
\def\Dz{$\dz$}
\def\Dt{\Delta t}
\def\Dz{\Delta z}
\def\dplus{D^+}
\def\Dp{$\dplus$}
\def\dzb{\overline{D}{}^0}
\def\Dzb{$\dzb$}
\def\dstl{\dstar\ell}
\def\dstpl{\dstarp\ell}
\def\dstzl{\dstarz\ell}
\def\dstml{\dstarm\ell}
\def\dstzbl{\dstarzb\ell}
\def\bdstlnu{\overline{B}\to\dstar\ell^-\nub}
\def\bdstxlnu{\overline{B}\to\dstar X\ell^-\nub}
\def\bzdstlnu{\bzb\to\dstarp\ell^-\nub}
\def\bzdstxlnu{\bzb\to\dstarp X\ell^-\nub}
\def\bmdstlnu{\bm\to\dstarz\ell^-\nub}
\def\bmdstxlnu{\bm\to\dstarz X\ell^-\nub}
\def\bmdstpxlnu{\bm\to\dstarp X\ell^-\nub}
\def\bpsik{\overline{B}\to\jpsi\kb}
\def\bdpi{\bbar\to D\pi}
\def\bzdstpm{\bzb\to\dstarp\pim}
\def\bzdstrhom{\bzb\to\dstarp\rhom}
\def\bzdppm{\bzb\to\dplus\pim}
\def\bmdzpm{\bm\to\dz\pim}
\def\bpsiks{B\to\jpsi\ks}
\def\bzbpsiks{\bzb\to\jpsi\ks}
\def\bzpsiks{\bz\to\jpsi\ks}
\def\bzbpsikst{\bzb\to\jpsi\kstarzb}
\def\bmpsikm{\bm\to\jpsi\km}
\def\nbdstlnu{N_{\bdstlnu}}
\def\nbdstxlnu{N_{\bdstxlnu}}
\def\nbb{N_{\bbbar}}
\def\ncc{N_{\ccbar}}
\def\kpi{K^-\pi^+}
\def\kpipiz{\km\pip\piz}
\def\kpipipi{\km\pip\pip\pim}
\def\kstarzb{\overline{K}{}^{*0}}
\def\Kstarzb{$\kstarzb$}
\def\UPS{$\Upsilon(4S)$}
\def\bgu{(\beta\gamma)_\Upsilon}
\def\pdstl{\mathbf{p}_{\dstar\ell}}
\def\pb{\mathbf{p}_{B}}
\def\Gevc{GeV/$c$}
\def\Gevcsq{GeV/$c^2$}
\def\Mevc{MeV/$c$}
\def\Mevcsq{MeV/$c^2$}
\def\degree{{}^{\rm o}}
\def\Degree{${}^{\rm o}$}
\def\dE{\Delta E}
\def\DE{$\dE$}
\def\mb{M_{\rm bc}}
\def\Mb{$\mb$}
\def\micron{$\mu$m}
\def\delz{\Delta z}
\def\delt{\Delta z}
\def\dt{\Delta t}
\def\dzb{\delz_B}
\def\dtb{\dt_B}
\def\dtp{\dt'}
\def\DTb{$\dtb$}
\def\dtrec{\dt_{rec}}
\def\dtgen{\dt_{gen}}
\def\dzrec{\delz_{rec}}
\def\dzgen{\delz_{gen}}
\def\sigdt{\sigma_{\dt}}
\def\sigpdt{\sigma'_{\dt}}
\def\sigmisdt{\sigma_{tail}^{\dt}}
\def\sigdz{\sigma_{\delz}}
\def\sigtdz{\tilde{\sigma}_{\delz}}
\def\sigtmisdz{\tilde{\sigma}_{tail}^{\delz}}
\def\arec{\alpha_{rec}}
\def\aasc{\alpha_{asc}}
\def\sigzrec{\sigma_{z}^{rec}}
\def\sigzasc{\sigma_{z}^{asc}}
\def\sigtzrec{\tilde{\sigma}_{z}^{rec}}
\def\sigtzasc{\tilde{\sigma}_{z}^{asc}}
\def\sigk{\sigma_{K}}
\def\sigmisk{\sigma_{tail}^{K}}
\def\smis{S_{tail}}
\def\scharm{S_{charm}}
\def\sdet{S_{det}}
% \def\sdata{S_{det}}
\def\sdata{s_{\rm data}}
\def\scmis{S_{tail}^{charm}}
\def\sdmis{S_{tail}^{det}}
\def\smisbg{S_{tail}^{\rm bkg}}
\def\sbg{S_{\rm bkg}}
\def\mudz{\mu_{\delz}}
\def\mumisdz{\mu_{tail}^{\delz}}
\def\mumisbg{\mu_{tail}^{\rm bkg}}
\def\muz{\mu_0}
\def\mumisz{\mu_{tail}^0}
\def\mudt{\mu_{\dt}}
\def\mumisdt{\mu_{tail}^{\dt}}
\def\amu{\alpha_\mu}
\def\amismu{\alpha_{tail}^{\mu}}
\def\mubg{\mu_{\rm bkg}}
\def\fmis{f_{tail}}
\def\fmisbg{f_{tail}^{\rm bkg}}
\def\flmbg{f_{\lambda \rm bkg}}
\def\fsig{f_{\rm sig}}
\def\fbkg{f_{\rm bkg}}
\def\fbg{f_{\rm bkg}}
\def\Fbg{F_{\rm bkg}}
\def\Fsig{F_{\rm sig}}
\def\lmbg{\lambda_{\rm bkg}}
\def\pbg{p_{\rm bkg}}
\def\fm{f_-}
\def\fz{f_0}
\def\ffdst{f_{f \dstar}}
\def\pfdst{p_{f \dstar}}
\def\lfdst{\lambda_{f \dstar}}
\def\ffl{f_{f \ell}}
\def\fbb{f_{\bbbar}}
\def\fcc{f_{\ccbar}}
\def\ftbg{f_{\tau {\rm bkg}}}
\def\frdstl{f_{R(\dstar\ell)}}
\def\fbgde{F_{\rm bkg}^{\dE}}
\def\fsigde{F_{\rm sig}^{\dE}}
\def\fbgmb{F_{\rm bkg}^{\mb}}
\def\fsigmb{F_{\rm sig}^{\mb}}
\def\rsig{R_{\rm sig}}
\def\rfdst{R_{f \dstar}}
\def\pfl{p_{f \ell}}
\def\pbb{p_{\bbbar}}
\def\pcc{p_{c\overline{c}}}
\def\Rsig{$\rsig$}
\def\rdz{R_{\delz}}
\def\rbg{R_{\rm bkg}}
\def\Rdz{$\rdz$}
\def\tbm{\tau_-}
\def\tbz{\tau_0}
\def\tsig{\tau_{\rm sig}}
\def\tbg{\tau_{\rm bkg}}
%\def\lfdst{{\cal L}_{f \dstar}}
\def\BF{{\cal B}}
\def\cosb{\cos\theta_B}
\def\ie{{\it i.e.}}
\def\psig{{{\cal P}_{\rm sig}}}
\def\pbkg{{{\cal P}_{\rm bkg}}}
\def\pasym{{{\cal P}_{\rm asym}}}
\def\rdet{{{R}_{\rm det}}}
\def\rnp{{{R}_{\rm np}}}
\def\rk{{{R}_{\rm k}}}


\newcommand{\Bcp}{B_{CP}}
\newcommand{\Btag}{B_{\rm tag}}
\newcommand{\zcp}{z_{CP}}
\newcommand{\ztag}{z_{\rm tag}}

\newcommand{\Brec}{B_{\rm rec}}
\newcommand{\Basc}{B_{\rm asc}}
\newcommand{\trec}{t_{\rm rec}}
\newcommand{\tasc}{t_{\rm asc}}
\newcommand{\zrec}{z_{\rm rec}}
\newcommand{\zasc}{z_{\rm asc}}
\newcommand{\Rrec}{R_{\rm rec}}
\newcommand{\Rasc}{R_{\rm asc}}
\newcommand{\Srec}{\sigma_{\rm rec}}
\newcommand{\Sasc}{\sigma_{\rm asc}}
\newcommand{\Scp}{\sigma_{CP}}
\newcommand{\Stag}{\sigma_{\rm tag}}
\newcommand{\Sdz}{\sigma_{\Dz}}
\newcommand{\Sdt}{\sigma_{\Dt}}

\newcommand{\tSdt}{\tilde{\sigma}_{\Dt}}
\newcommand{\tSdtm}{\tilde{\sigma}^{\Dt}_{\rm main}}
\newcommand{\tSdtt}{\tilde{\sigma}^{\Dt}_{\rm tail}}

\newcommand{\Sdtm}{\sigma^{\Dt}_{\rm main}}
\newcommand{\Mdtm}{\mu^{\Dt}_{\rm main}}
\newcommand{\Sdtt}{\sigma^{\Dt}_{\rm tail}}
\newcommand{\Mdtt}{\mu^{\Dt}_{\rm tail}}

\newcommand{\tScp}{\tilde{\sigma}_{CP}}
\newcommand{\tStag}{\tilde{\sigma}_{\rm tag}}
\newcommand{\tSdz}{\tilde{\sigma}_{\Dz}}
\newcommand{\tSdzm}{\tilde{\sigma}^{\Dz}_{\rm main}}
\newcommand{\tSdzt}{\tilde{\sigma}^{\Dz}_{\rm tail}}

\newcommand{\Sdzm}{\sigma^{\Dz}_{\rm main}}
\newcommand{\Mdzm}{\mu^{\Dz}_{\rm main}}
\newcommand{\Sdzt}{\sigma^{\Dz}_{\rm tail}}
\newcommand{\Mdzt}{\mu^{\Dz}_{\rm tail}}

\newcommand{\srec}{s_{\rm rec}}
\newcommand{\sasc}{s_{\rm asc}}

\newcommand{\sk}{\sigma_{\rm k}}
\newcommand{\snpm}{s_{\rm main}^{\rm NP}}
\newcommand{\snpt}{s_{\rm tail}^{\rm NP}}
\newcommand{\smain}{s_{\rm main}}
\newcommand{\stail}{s_{\rm tail}}
\newcommand{\ftail}{f_{\rm tail}}

% \newcommand{\bra}[1]{\left<#1\right|}
% \newcommand{\ket}[1]{\left|#1\right>}
\newcommand{\bra}[1]{\langle#1|}
\newcommand{\ket}[1]{|#1\rangle}
\newcommand{\braket}[2]{\langle#1|#2\rangle}
\newcommand{\rexp}[1]{{\rm e}^{#1}}
\newcommand{\ri}{{\rm i}}
\newcommand{\lcp}{{\lambda_{CP}}}
\newcommand{\dedx}{{\rm d}E/{\rm d}x}
\newcommand{\sinbb}{{\sin2\phi_1}}

\newcommand{\bcdot}{\!\cdot\!}

\def\dzp{\delz^\prime}
\def\fdelbg{f_\delta^{\rm bkg}}
\def\mudelbg{\mu_\delta^{\rm bkg}}
\def\mutaubg{\mu_\tau^{\rm bkg}}

\def\pol{p_{\rm ol}}
\def\fol{f_{\rm ol}}
\def\sigol{\sigma_{\rm ol}}




==> sensitivity_phi2/rhopi_dalitz.tex <==
\subsubsection{The prospect of $\phi_2$ using a full Dalitz plot analysis of $B^{0} \to \rho \pi \to \pi^+ \pi^- \pi^0$ decay}

The measurement of $\phi_2$  using isospin relation of $B \to \pi \pi$ decays has
ambiguity as we mention in Section\ref{sec:pipi2}.
Using a full Dalitz plot analysis of $B^{0} \to \rho \pi \to \pi^+ \pi^- \pi^0$ decay,
we can measure $\phi_2$ without this ambiguitiy\cite{bib:SQ-1993}.

Using the notation of Ref.~\cite{bib:phi2:LNQS}, 
the decay amplitudes of $B \to \rho\pi$ are expressed as
\begin{eqnarray}
 \sqrt{2}A(B^+\to \rho^+ \pi^0)&=&S_1=T^{+0}+2P_1,\\
 \sqrt{2}A(B^+\to \rho^0 \pi^+)&=&S_2=T^{0+}-2P_1,\\
 A(B^0\to \rho^+ \pi^-)&=&S_3=T^{+-}+P_1+P_0,\\
 A(B^0\to \rho^- \pi^+)&=&S_4=T^{-+}-P_1+P_0,\\
 A(B^0\to \rho^0 \pi^0)&=&S_5=T^{+0}+T^{0+}-T^{+-}-T^{-+}-2P_0.
\end{eqnarray}
Here $T^{ij}$ are the tree amplitudes where $i$ and $j$ are the $\rho$ and $\pi$
 charges, respectively.  $P_0$ and $P_1$ are the penguin amplitudes for $I = 0$ and
$I = 1$, respectively.
Similarly for the $CP$ conjugate channels, we define the amplitudes
$\bar{S}$, $\bar{T}^{ij}$, and $\bar{P}_i$ which differ from the
original amplitudes only in the sign of the weak phase of each term.
From isospin constraints, the following relation is hold for the above parameters:
\begin{eqnarray}
 S_1 + S_2 &=& S_3 + S_4 + S_5,\\
 \bar{S}_1 + \bar{S}_2 &=& \bar{S}_3 + \bar{S}_4 + \bar{S}_5.
\end{eqnarray}
%
In the full Dalitz plot analysis for the $\pi^+ \pi^- \pi^0$ final states,
we do not restrict what decay channels the $\pi^+ \pi^- \pi^0$ final states come from.
The amplitude of $B^0 \to \pi^+ \pi^- \pi^0$ decay is expressed as
\begin{equation}
 A(f) = f^+S_{3}+f^-S_{4}+f^0S_{5}/2,
\end{equation}
while the amplitude of the $CP$ conjugate channel is given by
\begin{equation}
 \bar{A}(f) = f^-\bar{S}_{3}+f^+\bar{S}_{4}+f^0\bar{S}_{5}/2.
\end{equation}
$f^i$ are the Breit-Wigner kinematic-distribution functions for
$\rho^{i}$ as described in the following formula:
\begin{equation}
 f(m, \theta) = \frac{\cos\theta\Gamma_{\rho}}
  {2(m_{\rho}-m-i0.5\Gamma_{\rho})},
\end{equation}
where $m_{\rho}$ and $\Gamma_{\rho}$ are the mass and width of $\rho$
meson, respectively.
%
The decay rate is given as the function of $\Delta t$, invariant mass $m_i$ and
helicity angle $\theta_i$ of $\rho$ by
%
\begin{eqnarray}
 \lefteqn{{\cal P}_{sig}(\Delta t, m_{+}, m_{-}, m_{0},
  \theta_{+}, \theta_{-}, \theta_{0})
  = \frac{e^{-|\Delta t|/\tau_{B^0}}}{4\tau_{B^0}}} \nonumber \\
 && \biggl[(|\bar{A}|^2+|A|^2)
  + q\left((\bar{|A|}^2-|A|^2)\cos(\Delta m \Delta t)
      +2\rm{Im}(\frac{\bar{A}}{A})\sin(\Delta m \Delta t)\right)
  \biggr]
\end{eqnarray}
where $q=1$ for $B_{tag}=B^0$ and $q=-1$ for $B_{tag}=\bar{B}^0$, and $i$ is the $\rho$ charge.
%
To clarify fit parameters, we denote $T^{ij}$ and $P_0$ as follows:
\begin{eqnarray}
 &&T=T^{+0}+T^{0+}=|T|e^{i\phi_3}e^{i\delta_{T}},\
  \bar{T}=\bar{T}^{+0}+\bar{T}^{0+}=|T|e^{-i\phi_3}e^{i\delta_{T}}\\
 &&T^{+-}=|T^{+-}|e^{i\phi_3}e^{i\delta_{+-}},\
  \bar{T}^{+-}=|T^{+-}|e^{-i\phi_3}e^{i\delta_{+-}}\\
 &&T^{-+}=|T^{-+}|e^{i\phi_3}e^{i\delta_{-+}},\
  \bar{T}^{-+}=|T^{-+}|e^{-i\phi_3}e^{i\delta_{-+}}\\
 &&P_{0}=|P_{0}|e^{-i\phi_1}e^{i\delta_{0}},\
  \bar{P}^{0}=|P_{0}|e^{i\phi_1}e^{i\delta_{0}}\\
 &&P_{1}=|P_{1}|e^{-i\phi_1}e^{i\delta_{1}},\
  \bar{P}^{1}=|P_{1}|e^{i\phi_1}e^{i\delta_{1}}
\end{eqnarray}
Here we use nine fit parameters as
\[
 \phi_2,\ |T|,\ \delta_{T},\ |T^{-+}|,\ \delta_{-+},
 \ |P_0|,\ \delta_0,\ |P_1|,\ \delta_1
\]
 and we set $|T^{+-}|=1,\ \delta_{+-}=0$.

We use the ensembles of the Monte Carlo(MC) pseudo-experiments for this study.
Each pseudo-experiment consists of events that are generated with the
nominal probability density functions (PDFs).
%
We generate only continuum background as background component at present.
Assuming $BR(B^0\to \rho \pi) = 25\times10^{-6}$ and the detection efficiency is 15\%,
we generate 10080 candidate events as data sample corresponding to 300fb$^{-1}$.
There are about 1240 signal event in this sample.
%
PDF for continuum background events is
%
\begin{eqnarray}
 {\cal P}_{q\overline{q}}
  =
  \frac{1}{2} {\cal M}(m_{+}, m_{-}, m_{0},
  \theta_{+}, \theta_{-}, \theta_{0})
  \Bigl\{f_\tau \frac{ e^{-|\Delta t|/\tau_{\rm bkg}} }{2\tau_{\rm bkg}}
  + ( 1 - f_\tau )\delta(\Delta t)\Bigl\},
  \label{phi2:eq:cont}
\end{eqnarray} 
where $f_{\tau}$ is the fraction of the background with effective lifetime
$\tau_{\rm bkg}$, $\delta$ is the Dirac delta function, and ${\cal M}$
is PDF in Dalitz plot plane for continuum background.
%
We define the likelihood value for each event as a function of 9
parameters:
%
\begin{eqnarray}
  \lefteqn{P_i(\Delta t_i,  m_{+}, m_{-}, m_{0},
  \theta_{+}, \theta_{-}, \theta_{0})) = 
%\nonumber \\
%& &
 (1 - f_{ol})\int^{+\infty}_{-\infty}
\{
(f_{sig}{\cal P}_{sig}(\Delta t^\prime, q, w_l)} \nonumber \\
 & &
  + f_{q\overline{q}}{\cal P}_{q\overline{q}}(\Delta t^\prime)
  \cdot R_{q\overline{q}}(\Delta t_i-\Delta t^\prime)\}
d\Delta t^\prime + f_{ol}{\cal P}_{ol}(\Delta{t_i}),
 \label{eq:Pevent}
\end{eqnarray}
where $f_{sig}$ and $f_{q\bar{q}}$ are the probability functions for signal events and
continuum background, respectively, and are determined on an event-by-event basis.
Signal fraction is estimated using data at the Belle experiment
by 2002 summer.
For signal events, we use the same values of resolution parameters as those
used for $\sin2\phi_1$ analysis.
We estimate the parameters for continuum background using the sideband data.

The input values of the fit parameters used here are listed in Table \ref{phi2:rptoymc_input} \cite{bib:phi2:PPP2003}.
%
\begin{table}
 \begin{center}
  \begin{tabular}{l|r||l|r}\hline \hline
   $\phi_2$ & \multicolumn{3}{l}{$1.57$  $(90 \deg)$} \\ \hline
   $|T|$ & $1.59$ & $\delta_T$ & $-0.65$ \\ \hline
   $|T^{+-}|$ & $1$ & $\delta_{T_{+-}}$ & $0$ \\ \hline
   $|T^{-+}|$ & $0.78$ & $\delta_{T_{-+}}$ & $-2.91$ \\ \hline
   $|P_{0}|$ & $0.19$ & $\delta_{P_{0}}$ & $-0.61$ \\ \hline
   $|P_{1}|$ & $0.19$ & $\delta_{P_{1}}$ & $1.04$ \\ \hline
  \end{tabular}
  \caption[The input parameters for full Dalitz plot analysis of $B^0 \to \pi^+ \pi^- \pi^0$ decay.]
{The input parameters for full Dalitz plot analysis of $B^0 \to \pi^+ \pi^- \pi^0$ decay.}
  \label{phi2:rptoymc_input}
 \end{center}
\end{table}
%
The result of the fit is shown in Figure \ref{phi2:fig:phi2err_rp}.
We obtain the $\phi_2$ error $\delta \phi_2 = 11.4 \deg$ for 300fb$^{-1}$ and $\delta \phi_2 = 3.5
\deg$ for 3ab$^{-1}$.
From these results, the error of $\phi_2$ is expected to be 2.9 $\deg$ for
5ab$^{-1}$ and 0.9 $\deg$ for 50ab$^{-1}$.

\begin{figure}
 \begin{center}
%  \includegraphics[width=8cm]{eps/phi2_err.eps}
  \includegraphics[width=8cm]{sensitivity_phi2/phi2_err.eps}
 \end{center}
 \caption[$\phi_2$ error as the function of luminosity.]
 {$\phi_2$ error as the function of luminosity. Dots are the results from the MC
 psuedo-experiments and the line is the linear fit to these dots.}
 \label{phi2:fig:phi2err_rp}
\end{figure}


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: t
%%% End: 


==> sensitivity_summary/figure.tex <==
}

